End-to-end Learning for OFDM: From Neural Receivers to Pilotless Communication

Previous studies have demonstrated that end-to-end learning enables significant shaping gains over additive white Gaussian noise (AWGN) channels. However, its benefits have not yet been quantified over realistic wireless channel models. This work aims to fill this gap by exploring the gains of end-to-end learning over a frequency- and time-selective fading channel using orthogonal frequency division multiplexing (OFDM). With imperfect channel knowledge at the receiver, the shaping gains observed on AWGN channels vanish. Nonetheless, we identify two other sources of performance improvements. The first comes from a neural network (NN)-based receiver operating over a large number of subcarriers and OFDM symbols which allows to significantly reduce the number of orthogonal pilots without loss of bit error rate (BER). The second comes from entirely eliminating orthognal pilots by jointly learning a neural receiver together with either superimposed pilots (SIPs), linearly combined with conventional quadrature amplitude modulation (QAM), or an optimized constellation geometry. The learned geometry works for a wide range of signal-to-noise ratios (SNRs), Doppler and delay spreads, has zero mean and does hence not contain any form of superimposed pilots. Both schemes achieve the same BER as the pilot-based baseline with around 7% higher throughput. Thus, we believe that a jointly learned transmitter and receiver are a very interesting component for beyond-5G communication systems which could remove the need and associated control overhead for demodulation reference signals (DMRSs).

==> figs/e2e_ber_gp_ds.tex <==
\begin{figure}
	\definecolor{C0}{HTML}{1F77B4}
	\definecolor{C1}{HTML}{FF7F0E}
	\definecolor{C2}{HTML}{2CA02C}
	\definecolor{C3}{HTML}{D62728}
	\definecolor{C4}{HTML}{9467BD}
	\definecolor{C5}{HTML}{8c564b}
	\definecolor{C6}{HTML}{e377c2}
	\definecolor{C7}{HTML}{7f7f7f}
 	\centering
 	\begin{subfigure}{1\linewidth}
 		\centering
		\begin{tikzpicture}
    		\begin{axis}[%
    			hide axis,
    			clip bounding box=upper bound,
    			legend style={draw=white!15!black,font=\footnotesize},
    			legend columns=3,
      			xmin=10,
    			xmax=10,
    			ymin=0,
    			ymax=0.1
    		]
    		\addlegendimage{C1,dashed, mark=diamond*}%
    		\addlegendentry{QAM \& Non-iterative 1P}%
   			\addlegendimage{C3,solid, mark=diamond*}%
    		\addlegendentry{QAM \& NN-based receiver 1P}%
    		\addlegendimage{C0,solid, mark=triangle*}%
    		\addlegendentry{QAM \& Perfect channel knowledge}%
        	\addlegendimage{C1,dashed, mark=square*}%
    		\addlegendentry{QAM \& Non-iterative 2P}%
    		\addlegendimage{C3,solid, mark=square*}%
    		\addlegendentry{QAM \& NN-based receiver 2P}%
    		\addlegendimage{C4,solid, mark=asterisk}%
    		\addlegendentry{GS \& Perfect channel knowledge}%    		
    		\addlegendimage{C5,solid, mark=*}%
       		\addlegendentry{GS \& NN-based receiver}%
     		\addlegendimage{C6,solid, mark=pentagon*}%
    		\addlegendentry{QAM \& SIP \& NN-based receiver}%

    		\end{axis}%
		\end{tikzpicture}
	\end{subfigure}
    \vspace{0.5\baselineskip}
	
 	\begin{subfigure}{0.45\linewidth}
 		\centering
		\begin{tikzpicture}[scale=0.8]
			\begin{semilogyaxis}[
				grid=both,
				grid style={line width=.4pt, draw=gray!10},
				major grid style={line width=.2pt,draw=gray!50},
				xlabel={$E_b/\sigma^2$ (dB)},
				ylabel={BER},
				xmax=18,
				xmin=5,
				ymax=0.5,
				ymin=1e-4,
			]
				\addplot[C3,solid, mark=diamond*] table [x=snr, y=ber, col sep=comma] {figs/qam_nnrx1p__ber_snr__ds_low.csv};
				\addplot[C5,solid, mark=*] table [x=snr, y=ber, col sep=comma] {figs/gs_nnrx__ber_snr__ds_low.csv};		
				\addplot[C0,solid, mark=triangle*] table [x=snr, y=ber, col sep=comma] {figs/qam_perfcsi__ber_snr__ds_low.csv};		
				\addplot[C3,solid, mark=square*] table [x=snr, y=ber, col sep=comma] {figs/qam_nnrx2p__ber_snr__ds_low.csv};		
				\addplot[C6,solid, mark=pentagon*] table [x=snr, y=ber, col sep=comma] {figs/qam_nnrxsip__ber_snr__ds_low.csv};		
				\addplot[C4,solid, mark=asterisk] table [x=snr, y=ber, col sep=comma] {figs/gs_perfcsi__ber_snr__ds_low.csv};	
				\end{semilogyaxis}	
			\end{tikzpicture}
    		\vspace{-0.4\baselineskip}
			\caption{BER at low delay spread}
	\end{subfigure}\quad\quad\quad
 	\begin{subfigure}{0.45\linewidth}
 		\centering
		\begin{tikzpicture}[scale=0.8]
			\begin{axis}[
    			clip bounding box=upper bound,
				grid=both,
				grid style={line width=.4pt, draw=gray!10},
				major grid style={line width=.2pt,draw=gray!50},
				%minor tick num=5,
				xlabel={$E_s/\sigma^2$ (dB)},
				ylabel={Goodput (bit/PRB)},
				xmax=25,
				xmin=5,
			]
				\addplot[C1,dashed, mark=diamond*] table [x=snr, y=goodput, col sep=comma] {figs/qam_lmmse1p__goodput_snr__ds_low.csv};
				\addplot[C3,solid, mark=diamond*] table [x=snr, y=goodput, col sep=comma] {figs/qam_nnrx1p__goodput_snr__ds_low.csv};
				\addplot[C5,solid, mark=*] table [x=snr, y=goodput, col sep=comma] {figs/gs_nnrx__goodput_snr__ds_low.csv};		
				\addplot[C0,solid, mark=triangle*] table [x=snr, y=goodput, col sep=comma] {figs/qam_perfcsi__goodput_snr__ds_low.csv};		
				\addplot[C1,dashed, mark=square*] table [x=snr, y=goodput, col sep=comma] {figs/qam_lmmse2p__goodput_snr__ds_low.csv};
				\addplot[C3,solid, mark=square*] table [x=snr, y=goodput, col sep=comma] {figs/qam_nnrx2p__goodput_snr__ds_low.csv};	
				\addplot[C6,solid, mark=pentagon*] table [x=snr, y=goodput, col sep=comma] {figs/qam_nnrxsip__goodput_snr__ds_low.csv};		
				\addplot[C4,solid, mark=asterisk] table [x=snr, y=goodput, col sep=comma] {figs/gs_perfcsi__goodput_snr__ds_low.csv};	
				\end{axis}	
			\end{tikzpicture}
    		\vspace{-0.4\baselineskip}
			\caption{Goodput at low delay spread}
	\end{subfigure}
    \vspace{0.3\baselineskip}
	
 	\begin{subfigure}{0.45\linewidth}
 		\centering
		\begin{tikzpicture}[scale=0.8]
			\begin{semilogyaxis}[
    			clip bounding box=upper bound,
				grid=both,
				grid style={line width=.4pt, draw=gray!10},
				major grid style={line width=.2pt,draw=gray!50},
				xlabel={$E_b/\sigma^2$ (dB)},
				ylabel={BER},
				xmax=18,
				xmin=5,
				ymax=0.5,
				ymin=1e-4,
			]
				\addplot[C3,dashed, mark=diamond*] table [x=snr, y=ber, col sep=comma] {figs/qam_nnrx1p__ber_snr__ds_med.csv};		
				\addplot[C5,solid, mark=*] table [x=snr, y=ber, col sep=comma] {figs/gs_nnrx__ber_snr__ds_med.csv};		
				\addplot[C0,solid, mark=triangle*] table [x=snr, y=ber, col sep=comma] {figs/qam_perfcsi__ber_snr__ds_med.csv};		
				\addplot[C3,dashed, mark=square*] table [x=snr, y=ber, col sep=comma] {figs/qam_nnrx2p__ber_snr__ds_med.csv};		
				\addplot[C6,solid, mark=pentagon*] table [x=snr, y=ber, col sep=comma] {figs/qam_nnrxsip__ber_snr__ds_med.csv};		
				\addplot[C4,solid, mark=asterisk] table [x=snr, y=ber, col sep=comma] {figs/gs_perfcsi__ber_snr__ds_med.csv};	
				\end{semilogyaxis}	
			\end{tikzpicture}
    		\vspace{-0.4\baselineskip}
			\caption{BER at medium delay spread}
	\end{subfigure}\quad\quad\quad
 	\begin{subfigure}{0.45\linewidth}
 		\centering
		\begin{tikzpicture}[scale=0.8]
			\begin{axis}[
    			clip bounding box=upper bound,
				grid=both,
				grid style={line width=.4pt, draw=gray!10},
				major grid style={line width=.2pt,draw=gray!50},
				%minor tick num=5,
				xlabel={$E_s/\sigma^2$ (dB)},
				ylabel={Goodput (bit/PRB)},
				xmax=25,
				xmin=5,
			]
				\addplot[C1,dashed, mark=diamond*] table [x=snr, y=goodput, col sep=comma] {figs/qam_lmmse1p__goodput_snr__ds_med.csv};	
				\addplot[C3,solid, mark=diamond*] table [x=snr, y=goodput, col sep=comma] {figs/qam_nnrx1p__goodput_snr__ds_med.csv};	
				\addplot[C5,solid, mark=*] table [x=snr, y=goodput, col sep=comma] {figs/gs_nnrx__goodput_snr__ds_med.csv};		
				\addplot[C0,solid, mark=triangle*] table [x=snr, y=goodput, col sep=comma] {figs/qam_perfcsi__goodput_snr__ds_med.csv};		
				\addplot[C1,dashed, mark=square*] table [x=snr, y=goodput, col sep=comma] {figs/qam_lmmse2p__goodput_snr__ds_med.csv};
				\addplot[C3,solid, mark=square*] table [x=snr, y=goodput, col sep=comma] {figs/qam_nnrx2p__goodput_snr__ds_med.csv};	
				\addplot[C6,solid, mark=pentagon*] table [x=snr, y=goodput, col sep=comma] {figs/qam_nnrxsip__goodput_snr__ds_med.csv};		
				\addplot[C4,solid, mark=asterisk] table [x=snr, y=goodput, col sep=comma] {figs/gs_perfcsi__goodput_snr__ds_med.csv};		
				\end{axis}	
			\end{tikzpicture}
    		\vspace{-0.4\baselineskip}
			\caption{Goodput at medium delay spread}
	\end{subfigure}
    \vspace{0.3\baselineskip}
	
 	\begin{subfigure}{0.45\linewidth}
 		\centering
		\begin{tikzpicture}[scale=0.8]
			\begin{semilogyaxis}[
    			clip bounding box=upper bound,
				grid=both,
				grid style={line width=.4pt, draw=gray!10},
				major grid style={line width=.2pt,draw=gray!50},
				xlabel={$E_b/\sigma^2$ (dB)},
				ylabel={BER},
				xmax=18,
				xmin=5,
				ymax=0.5,
				ymin=1e-4,
			]
				\addplot[C3,dashed, mark=diamond*] table [x=snr, y=ber, col sep=comma] {figs/qam_nnrx1p__ber_snr__ds_high.csv};		
				\addplot[C5,solid, mark=*] table [x=snr, y=ber, col sep=comma] {figs/gs_nnrx__ber_snr__ds_high.csv};		
				\addplot[C0,solid, mark=triangle*] table [x=snr, y=ber, col sep=comma] {figs/qam_perfcsi__ber_snr__ds_high.csv};		
				\addplot[C3,dashed, mark=square*] table [x=snr, y=ber, col sep=comma] {figs/qam_nnrx2p__ber_snr__ds_high.csv};		
				\addplot[C6,solid, mark=pentagon*] table [x=snr, y=ber, col sep=comma] {figs/qam_nnrxsip__ber_snr__ds_high.csv};		
				\addplot[C4,solid, mark=asterisk] table [x=snr, y=ber, col sep=comma] {figs/gs_perfcsi__ber_snr__ds_high.csv};	
				\end{semilogyaxis}	
			\end{tikzpicture}
    		\vspace{-0.4\baselineskip}
			\caption{BER at high delay spread}
	\end{subfigure}\quad\quad\quad
 	\begin{subfigure}{0.45\linewidth}
 		\centering
		\begin{tikzpicture}[scale=0.8]
			\begin{axis}[
    			clip bounding box=upper bound,
				grid=both,
				grid style={line width=.4pt, draw=gray!10},
				major grid style={line width=.2pt,draw=gray!50},
				%minor tick num=5,
				xlabel={$E_s/\sigma^2$ (dB)},
				ylabel={Goodput (bit/PRB)},
				xmax=25,
				xmin=5,
			]		
				\addplot[C1,dashed, mark=diamond*] table [x=snr, y=goodput, col sep=comma] {figs/qam_lmmse1p__goodput_snr__ds_high.csv};
				\addplot[C3,solid, mark=diamond*] table [x=snr, y=goodput, col sep=comma] {figs/qam_nnrx1p__goodput_snr__ds_high.csv};
				\addplot[C5,solid, mark=*] table [x=snr, y=goodput, col sep=comma] {figs/gs_nnrx__goodput_snr__ds_high.csv};		
				\addplot[C0,solid, mark=triangle*] table [x=snr, y=goodput, col sep=comma] {figs/qam_perfcsi__goodput_snr__ds_high.csv};
				\addplot[C1,dashed, mark=square*] table [x=snr, y=goodput, col sep=comma] {figs/qam_lmmse2p__goodput_snr__ds_high.csv};
				\addplot[C3,solid, mark=square*] table [x=snr, y=goodput, col sep=comma] {figs/qam_nnrx2p__goodput_snr__ds_high.csv};	
				\addplot[C6,solid, mark=pentagon*] table [x=snr, y=goodput, col sep=comma] {figs/qam_nnrxsip__goodput_snr__ds_high.csv};		
				\addplot[C4,solid, mark=asterisk] table [x=snr, y=goodput, col sep=comma] {figs/gs_perfcsi__goodput_snr__ds_high.csv};	
				\end{axis}	
			\end{tikzpicture}
    		\vspace{-0.4\baselineskip}
			\caption{Goodput at high delay spread}
	\end{subfigure}
	\caption{BER and goodput achieved by the evaluated schemes for different ranges of delay spread. The low speed range is considered.\label{fig:e2e_ber_gp_ds}}
\end{figure}


==> figs/rx_ber_ds.tex <==
\begin{figure}
	\definecolor{C0}{HTML}{1F77B4}
	\definecolor{C1}{HTML}{FF7F0E}
	\definecolor{C2}{HTML}{2CA02C}
	\definecolor{C3}{HTML}{D62728}
	\definecolor{C4}{HTML}{9467BD}
 	\centering
 	\begin{subfigure}{1\linewidth}
 		\centering
		\begin{tikzpicture}
    		\begin{axis}[%
    			hide axis,
    			clip bounding box=upper bound,
    			legend style={draw=white!15!black,font=\footnotesize},
    			legend columns=4,
      			xmin=10,
    			xmax=10,
    			ymin=0,
    			ymax=0.1
    		]
    		\addlegendimage{C1,dashed, mark=diamond*}%
    		\addlegendentry{Non-iterative 1P}%
   			\addlegendimage{C2,dotted, mark=diamond*}%
    		\addlegendentry{Iterative 1P}%
   			\addlegendimage{C3,solid, mark=diamond*}%
    		\addlegendentry{NN-based receiver 1P}%
    		\addlegendimage{C0,solid, mark=triangle*}%
    		\addlegendentry{Perfect channel knowledge}%
    		\addlegendimage{C1,dashed, mark=square*}%
    		\addlegendentry{Non-iterative 2P}%
    		\addlegendimage{C2,dotted, mark=square*}%
    		\addlegendentry{Iterative 2P}%
    		\addlegendimage{C3,solid, mark=square*}%
    		\addlegendentry{NN-based receiver 2P}%
    		\end{axis}%
		\end{tikzpicture}
	\end{subfigure}
    \vspace{0.5\baselineskip}
	
 	\begin{subfigure}{0.45\linewidth}
 		\centering
		\begin{tikzpicture}[scale=0.8]
			\begin{semilogyaxis}[
				grid=both,
				grid style={line width=.4pt, draw=gray!10},
				major grid style={line width=.2pt,draw=gray!50},
				xlabel={$E_b/\sigma^2$ (dB)},
				ylabel={BER},
				xmax=18,
				xmin=5,
				ymax=0.5,
				ymin=1e-4,
			]
				\addplot[C1,dashed, mark=diamond*] table [x=snr, y=ber, col sep=comma] {figs/qam_lmmse1p__ber_snr__ds_low.csv};		
				\addplot[C2,dotted, mark=diamond*] table [x=snr, y=ber, col sep=comma] {figs/qam_idd1p__ber_snr__ds_low.csv};		
				\addplot[C3,solid, mark=diamond*] table [x=snr, y=ber, col sep=comma] {figs/qam_nnrx1p__ber_snr__ds_low.csv};		
				\addplot[C0,solid, mark=triangle*] table [x=snr, y=ber, col sep=comma] {figs/qam_perfcsi__ber_snr__ds_low.csv};			
				\end{semilogyaxis}	
			\end{tikzpicture}
    		\vspace{-0.4\baselineskip}
			\caption{1P pilot pattern at low delay spread range}
	\end{subfigure}\quad\quad\quad
 	\begin{subfigure}{0.45\linewidth}
 		\centering
		\begin{tikzpicture}[scale=0.8]
			\begin{semilogyaxis}[
    			clip bounding box=upper bound,
				grid=both,
				grid style={line width=.4pt, draw=gray!10},
				major grid style={line width=.2pt,draw=gray!50},
				%minor tick num=5,
				xlabel={$E_b/\sigma^2$ (dB)},
				ylabel={BER},
				xmax=18,
				xmin=5,
				ymax=0.5,
				ymin=1e-4,
			]
				\addplot[C1,dashed, mark=square*] table [x=snr, y=ber, col sep=comma] {figs/qam_lmmse2p__ber_snr__ds_low.csv};
				\addplot[C2,dotted, mark=square*] table [x=snr, y=ber, col sep=comma] {figs/qam_idd2p__ber_snr__ds_low.csv};			
				\addplot[C3,solid, mark=square*] table [x=snr, y=ber, col sep=comma] {figs/qam_nnrx2p__ber_snr__ds_low.csv};		
				\addplot[C0,solid, mark=triangle*] table [x=snr, y=ber, col sep=comma] {figs/qam_perfcsi__ber_snr__ds_low.csv};			
				\end{semilogyaxis}	
			\end{tikzpicture}
    		\vspace{-0.4\baselineskip}
			\caption{2P pilot pattern at low delay spread range}
	\end{subfigure}
    \vspace{0.3\baselineskip}
	
 	\begin{subfigure}{0.45\linewidth}
 		\centering
		\begin{tikzpicture}[scale=0.8]
			\begin{semilogyaxis}[
    			clip bounding box=upper bound,
				grid=both,
				grid style={line width=.4pt, draw=gray!10},
				major grid style={line width=.2pt,draw=gray!50},
				xlabel={$E_b/\sigma^2$ (dB)},
				ylabel={BER},
				xmax=18,
				xmin=5,
				ymax=0.5,
				ymin=1e-4,
			]
				\addplot[C1,dashed, mark=diamond*] table [x=snr, y=ber, col sep=comma] {figs/qam_lmmse1p__ber_snr__ds_med.csv};		
				\addplot[C2,dotted, mark=diamond*] table [x=snr, y=ber, col sep=comma] {figs/qam_idd1p__ber_snr__ds_med.csv};		
				\addplot[C3,solid, mark=diamond*] table [x=snr, y=ber, col sep=comma] {figs/qam_nnrx1p__ber_snr__ds_med.csv};		
				\addplot[C0,solid, mark=triangle*] table [x=snr, y=ber, col sep=comma] {figs/qam_perfcsi__ber_snr__ds_med.csv};			
				\end{semilogyaxis}	
			\end{tikzpicture}
    		\vspace{-0.4\baselineskip}
			\caption{1P pilot pattern at medium delay spread}
	\end{subfigure}\quad\quad\quad
 	\begin{subfigure}{0.45\linewidth}
 		\centering
		\begin{tikzpicture}[scale=0.8]
			\begin{semilogyaxis}[
    			clip bounding box=upper bound,
				grid=both,
				grid style={line width=.4pt, draw=gray!10},
				major grid style={line width=.2pt,draw=gray!50},
				%minor tick num=5,
				xlabel={$E_b/\sigma^2$ (dB)},
				ylabel={BER},
				xmax=18,
				xmin=5,
				ymax=0.5,
				ymin=1e-4,
			]
				\addplot[C1,dashed, mark=square*] table [x=snr, y=ber, col sep=comma] {figs/qam_lmmse2p__ber_snr__ds_med.csv};		
				\addplot[C2,dotted, mark=square*] table [x=snr, y=ber, col sep=comma] {figs/qam_idd2p__ber_snr__ds_med.csv};			
				\addplot[C3,solid, mark=square*] table [x=snr, y=ber, col sep=comma] {figs/qam_nnrx2p__ber_snr__ds_med.csv};		
				\addplot[C0,solid, mark=triangle*] table [x=snr, y=ber, col sep=comma] {figs/qam_perfcsi__ber_snr__ds_med.csv};			
				\end{semilogyaxis}	
			\end{tikzpicture}
    		\vspace{-0.4\baselineskip}
			\caption{2P pilot pattern at medium delay spread}
	\end{subfigure}
    \vspace{0.3\baselineskip}
	
 	\begin{subfigure}{0.45\linewidth}
 		\centering
		\begin{tikzpicture}[scale=0.8]
			\begin{semilogyaxis}[
    			clip bounding box=upper bound,
				grid=both,
				grid style={line width=.4pt, draw=gray!10},
				major grid style={line width=.2pt,draw=gray!50},
				xlabel={$E_b/\sigma^2$ (dB)},
				ylabel={BER},
				xmax=18,
				xmin=5,
				ymax=0.5,
				ymin=1e-4,
			]
				\addplot[C1,dashed, mark=diamond*] table [x=snr, y=ber, col sep=comma] {figs/qam_lmmse1p__ber_snr__ds_high.csv};		
				\addplot[C2,dotted, mark=diamond*] table [x=snr, y=ber, col sep=comma] {figs/qam_idd1p__ber_snr__ds_high.csv};		
				\addplot[C3,solid, mark=diamond*] table [x=snr, y=ber, col sep=comma] {figs/qam_nnrx1p__ber_snr__ds_high.csv};		
				\addplot[C0,solid, mark=triangle*] table [x=snr, y=ber, col sep=comma] {figs/qam_perfcsi__ber_snr__ds_high.csv};			
				\end{semilogyaxis}	
			\end{tikzpicture}
    		\vspace{-0.4\baselineskip}
			\caption{1P pilot pattern at high delay spreads}
	\end{subfigure}\quad\quad\quad
 	\begin{subfigure}{0.45\linewidth}
 		\centering
		\begin{tikzpicture}[scale=0.8]
			\begin{semilogyaxis}[
    			clip bounding box=upper bound,
				grid=both,
				grid style={line width=.4pt, draw=gray!10},
				major grid style={line width=.2pt,draw=gray!50},
				%minor tick num=5,
				xlabel={$E_b/\sigma^2$ (dB)},
				ylabel={BER},
				xmax=18,
				xmin=5,
				ymax=0.5,
				ymin=1e-4,
			]		
				\addplot[C1,dashed, mark=square*] table [x=snr, y=ber, col sep=comma] {figs/qam_lmmse2p__ber_snr__ds_high.csv};		
				\addplot[C2,dotted, mark=square*] table [x=snr, y=ber, col sep=comma] {figs/qam_idd2p__ber_snr__ds_high.csv};		
				\addplot[C3,solid, mark=square*] table [x=snr, y=ber, col sep=comma] {figs/qam_nnrx2p__ber_snr__ds_high.csv};		
				\addplot[C0,solid, mark=triangle*] table [x=snr, y=ber, col sep=comma] {figs/qam_perfcsi__ber_snr__ds_high.csv};			

				\end{semilogyaxis}	
			\end{tikzpicture}
    		\vspace{-0.4\baselineskip}
			\caption{2P pilot pattern at high delay spread}
	\end{subfigure}
	\caption{BER achieved by the evaluated receivers for different ranges of delay spread. The low speed range is considered.\label{fig:rx_ber_ds}}
\end{figure}

